Selective Off-Policy Reference Tuning with Plan Guidance

Reinforcement learning with verifiable rewards helps reasoning, but GRPO-style methods stall on hard prompts where all sampled rollouts fail. SORT adds a repair update for those failures without changing rollout generation: it derives a plan from the reference solution, compares token probabilities with and without that plan, and gives higher weight to tokens that become more predictable under plan conditioning. This turns all-wrong prompts into selective, structure-aware learning signals instead of uniform imitation. Across three backbones and eight reasoning benchmarks, SORT improves over GRPO and guidance baselines, with largest gains on weaker models.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., ``error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction claim that SORT repairs zero-reward GRPO prompts via plan-conditioned token-selective reference updates without altering rollout generation, and that it improves over GRPO and guidance-based baselines across multiple backbones. These claims are directly supported by the main benchmark results (Table~1), training dynamics (Figure~1), ablation studies (Tables~2--3), and the theoretical regret bound (Theorem~1).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~A provides a dedicated ``Limitations \& Broader Impacts'' section that discusses five limitations: dependence on verified reference solutions, plan extraction quality tied to model capability, additional compute overhead from auxiliary updates, evaluation restricted to math and knowledge benchmarks, and absence of multi-seed error bars. Theorem~1 also bounds the weight approximation error by the plan quality parameter~$\gamma$.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: All theoretical results are stated with their required assumptions (Assumptions~1--2 in Section~3.4), and complete proofs of Lemma~1 and Theorem~1 are provided in Appendix~G. Definitions~1--2 in Section~3.2 give the formal setup. Theorem~1 is cross-referenced and its proof details the derivation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~4.1 specifies all model versions (Llama-3.2-3B-Instruct, Qwen2.5-7B-Instruct, Qwen3-4B-Instruct), the training dataset (OpenR1-Math-220k subset with 15k prompts), the full optimization configuration (verl + vLLM, 8~A100 GPUs, $\beta_{\text{KL}}=0$, asymmetric clipping $\epsilon_{\text{low}}=0.2$ / $\epsilon_{\text{high}}=0.28$, batch size~128, 8~trajectories per prompt, 500~steps, max length~8096), the evaluation protocol (avg@16), and all eight benchmarks. Algorithm~1 in Appendix~A gives the complete SORT procedure, and Appendix~E provides prompt templates.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable.
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The training code and experiment scripts are submitted alongside the paper as anonymized supplemental material, with instructions for reproducing the main results. The training data (OpenR1-Math-220k subset of NuminaMath~1.5~\citep{li2024numinamath}) and all evaluation benchmarks (AIME24/25, AMC23, MATH-500, Minerva Math, OlympiadBench, GPQA, MMLU-Pro) are publicly available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~4.1 provides the complete experimental configuration: model versions, dataset (15k OpenR1-Math-220k subset), optimizer setup (verl + vLLM, AdamW), hyperparameters ($\beta_{\text{KL}}=0$, $\epsilon_{\text{low}}=0.2$, $\epsilon_{\text{high}}=0.28$, batch~128, 8~rollouts/prompt, 500~steps, max length~8096), and evaluation protocol (avg@16 across eight benchmarks). Hyperparameters follow standard RLVR practice~\citep{dapo,grpo} and the same settings are used for all baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Table~1--3 results are reported as avg@16 point estimates without error bars, standard deviations, or formal statistical significance tests over multiple training runs. The consistent improvement pattern across three model scales (Llama-3.2-3B, Qwen2.5-7B, Qwen3-4B) and eight benchmarks makes random noise an unlikely explanation, and the trends are stable across training steps (Figure~1). We acknowledge this limitation in Appendix~A and note that reporting multi-seed variance would further strengthen the empirical claims.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~4.1 specifies 8~A100 GPUs per training run with verl for optimization and vLLM for sampling. Each method trains for 500~steps with batch size~128 and 8~trajectories per prompt at max length~8096. Approximate wall-clock time per run is \textasciitilde{}18--24~hours on 8~A100s depending on the backbone size. The full project, including preliminary runs and baselines, used roughly 4--5$\times$ the compute reported for the final experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics. This work does not involve human subjects, crowdsourcing, personally identifiable data, or downstream applications with direct fairness or privacy concerns. All datasets and models used are publicly available and properly cited. The submission preserves anonymity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~A includes a ``Broader impacts'' paragraph discussing positive impacts (improved sample efficiency for RLVR training, reduced compute costs, applicability to theorem proving and scientific reasoning) and potential negative impacts (lowering the barrier for fine-tuning stronger reasoning capabilities, which could aid misuse such as automated vulnerability discovery). We note this risk is shared by all LLM reasoning improvements and is not specific to SORT, and we encourage standard responsible-release practices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not release new pre-trained models, image generators, scraped datasets, or other assets that carry high risk for misuse. The paper proposes a training algorithm; no new high-risk artifacts are introduced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNo{}
    \item[] Justification: All models (Llama-3.2-3B-Instruct, Qwen2.5-7B-Instruct, Qwen3-4B-Instruct) and datasets (OpenR1-Math-220k, AIME, AMC, MATH-500, Minerva Math, OlympiadBench, GPQA, MMLU-Pro) are cited with their original references, and we respect their terms of use. However, the specific license names (e.g., Llama~3.2 Community License, Qwen License, Apache~2.0, CC-BY~4.0, MIT) are not explicitly listed in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not introduce new datasets, models, or other assets. The submitted anonymized code is documented with a README and reproduction instructions, but the core contribution is an algorithmic method, not a released asset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work does not involve crowdsourcing experiments or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work does not involve human subjects research and therefore does not require IRB approval.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are the subject of study in this work (we train Llama and Qwen models), not a component of the core methodology. The plan extraction step uses the same model being optimized, not an external LLM. No external LLM is used for data generation, evaluation, or any other methodological purpose.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> sections/background.tex <==
\section{Preliminaries}
\label{sec:prelim}

\paragraph{Problem setting.}
We consider a dataset $\mathcal{D}=\{(q_i,y_i^\star)\}$ of mathematical reasoning problems, where $q_i$ is a prompt and $y_i^\star$ is a verified reference solution with an automatically checkable final answer. Training uses binary verifiable rewards, and the goal is to improve the policy $\pi_\theta$ while preserving generalization to held-out and out-of-distribution benchmarks.

\paragraph{GRPO and all-wrong collapse.}
For a prompt $x$, GRPO samples $G$ rollouts $\{y_i\}_{i=1}^G \sim \pi_{\theta_{\mathrm{old}}}(\cdot\mid x)$ and receives binary verifiable rewards $r_i\in\{0,1\}$. It computes group-relative advantages
\begin{equation}
\bar r = \frac{1}{G}\sum_{j=1}^G r_j,\qquad
\sigma_r = \sqrt{\frac{1}{G}\sum_{j=1}^G (r_j-\bar r)^2},\qquad
A_i = \frac{r_i-\bar r}{\sigma_r+\epsilon}.
\end{equation}
The policy-gradient contribution of each rollout is proportional to $A_i$ \citep{grpo,dapo}. Hence, when all rollouts are incorrect,
\begin{equation}
r_1=\cdots=r_G=0
\;\Longrightarrow\;
A_i=0\ \forall i
\;\Longrightarrow\;
\nabla_\theta \mathcal{L}_{\mathrm{GRPO}}=0.
\end{equation}
The prompt contributes no learning signal, even though its verified reference solution $y^\star$ is available.

\paragraph{Reference-path weighting.}
For a verified reference $y^\star=(y_1^\star,\dots,y_T^\star)$, write
\begin{equation}
p_S^t := \pi_\theta(y_t^\star \mid y_{<t}^\star,x).
\end{equation}
Standard reference imitation minimizes $-\sum_t\log p_S^t$, assigning the same likelihood objective to every token. On hard references this can be unstable, because very low-probability tokens can dominate the update. Dynamic Fine-Tuning (DFT) instead uses the detached student probability as a support-aware weight,
\begin{equation}
\mathcal{L}_{\mathrm{DFT}}
=
-\sum_t \operatorname{sg}(p_S^t)\log p_S^t,
\end{equation}
where $\operatorname{sg}(\cdot)$ denotes stop-gradient \citep{wu2026generalizationsftreinforcementlearning}.


==> sections/methodology_phat.tex <==
\section{Method}
\label{sec:method}

We propose \textbf{Selective Off-Policy Learning via Self-Distillation (SOLD)}, an auxiliary repair mechanism for the zero-reward regime of GRPO. The main GRPO rollout process is left unchanged.

\subsection{From Zero-Reward Failures to Deferred Repair}

Consider a GRPO training iteration with rollout batch $\mathcal{U}_k = \{q_i\}_{i=1}^{B_{\mathrm{rl}}}$. For each prompt $q_i$, the model samples $N$ responses and receives binary verifiable rewards. When every rollout is incorrect, the group-relative advantage collapses to zero and the prompt contributes no gradient. These \emph{zero-reward prompts},
\begin{equation}
\mathcal{I}_{\mathrm{aw}}^{(k)} = \{ i : r_i^{(n)} = 0,\; \forall n \in [N] \},
\label{eq:aw_index}
\end{equation}
are not noise---they are the hard cases where the model most needs to improve. A prompt ends up in this regime because the model fails to produce the key reasoning steps (derivative $\to$ solve $\to$ classify) that structure a correct solution. Yet each such prompt has a verified reference $y_i^\star$ that contains exactly those steps, just interleaved with surface details (numbers, expansions, wording). The bottleneck is not a lack of supervision, but a lack of \emph{selectivity}: without knowing which tokens encode the missing reasoning, uniform imitation of the full reference harms generalization \citep{wu2026generalizationsftreinforcementlearning}.

SOLD resolves this by deferring repair. Failed prompts are neither skipped nor merged into GRPO; they are \textbf{buffered} for a separate auxiliary update:
\begin{equation}
\mathcal{B}_{\mathrm{aw}} \leftarrow \operatorname{Enqueue}\!\bigl(\mathcal{B}_{\mathrm{aw}},\; \{(q_i, y_i^\star) : i \in \mathcal{I}_{\mathrm{aw}}^{(k)}\}\bigr).
\label{eq:enqueue}
\end{equation}
When $|\mathcal{B}_{\mathrm{aw}}| \ge B_{\mathrm{aux}}$, a minibatch $\mathcal{M}_k \sim \operatorname{SampleBatch}(\mathcal{B}_{\mathrm{aw}}, B_{\mathrm{aux}})$ triggers one SOLD update. GRPO continues learning from prompts with reward variance; SOLD repairs the hard frontier.

\subsection{Identifying Reasoning-Critical Tokens via Plan Conditioning}

Once a buffered prompt enters the auxiliary update, the core question is: \emph{which tokens} in $y_i^\star$ encode the reasoning logic, as opposed to surface wording, formatting, or routine algebra? We first define what makes a token reasoning-critical, then show how to detect such tokens operationally.

\begin{definition}[Latent reasoning plan]
\label{def:latent_plan}
Human problem solving proceeds in two stages: first form a high-level \emph{reasoning plan} $S$ (key steps, transformations, decisions), then render it into a detailed solution $y^\star$. Formally, the model's predictive distribution marginalizes over possible plans:
\begin{equation}
\pi_\theta(y_t^\star \mid y_{<t}^\star, q)
= \int \pi_\theta(y_t^\star \mid S, y_{<t}^\star, q)\; dP(S \mid y_{<t}^\star, q).
\label{eq:plan_marginal}
\end{equation}
The plan $S$ is not observed---only the full solution $y^\star$ is available.
\end{definition}

\begin{definition}[Structural salience]
\label{def:structural_token}
The \emph{structural salience} of token $y_t^\star$ is the pointwise mutual information between the plan $S$ and the token:
\begin{equation}
\sigma_t \;:=\; \log \frac{\pi_\theta(y_t^\star \mid S, y_{<t}^\star, q)}{\pi_\theta(y_t^\star \mid y_{<t}^\star, q)}.
\label{eq:sigma_def}
\end{equation}
$\sigma_t > 0$ means knowing $S$ makes the token more predictable (e.g., ``$f'(x)=3x^2-3$'' after being told to differentiate); $\sigma_t \approx 0$ means the token is independent of the plan (formatting, boilerplate). This operational definition requires no external labels.
\end{definition}

Definitions~\ref{def:latent_plan}--\ref{def:structural_token} give us a target: if we had access to the true plan $S$, the salience $\sigma_t$ would tell us exactly how much to emphasize each token. Since $S$ is latent, SOLD approximates $\sigma_t$ through three operational steps.

\paragraph{Step 1: Extract a solution blueprint.}
We estimate $S$ by prompting the model to extract the reasoning structure from the reference solution---the key steps, decisions, and intermediate realizations that constitute the solution's logical core:
\begin{equation}
\hat{y}_i = \operatorname{Gen}_\theta\!\bigl(\textsc{SkelPrompt}(q_i, y_i^\star)\bigr).
\label{eq:blueprint}
\end{equation}
Unlike the full reference, which interleaves structural reasoning with surface realization (specific numbers, algebraic expansions, formatting), the blueprint isolates the \emph{thinking process}: for a calculus problem whose reference expands ``$f'(x) = 3x^2 - 6x + 2$, setting $f'(x)=0$ and applying the quadratic formula yields $x = 1 \pm \sqrt{3}/3$'', the blueprint extracts the underlying plan: ``Compute derivative, solve $f'(x)=0$ via quadratic formula, classify via second derivative test.'' The blueprint need not be short; it should faithfully capture the reasoning structure. Prompt templates are in Appendix~\ref{app:prompt_templates}.

\paragraph{Step 2: Score the reference under two prefixes.}
We evaluate the model on the \emph{same reference sequence} $y_i^\star$ under two prefixes that differ only in whether the blueprint is provided:
\begin{align}
\text{Student:}\quad
p_S^t &= \pi_\theta\bigl(y_{i,t}^\star \mid \textsc{StudentPrompt}(q_i),\, y_{i,<t}^\star\bigr), \\[4pt]
\text{Teacher:}\quad
p_T^t &= \pi_\theta\bigl(y_{i,t}^\star \mid \textsc{TeacherPrompt}(q_i, \hat{y}_i),\, y_{i,<t}^\star\bigr),
\end{align}
where $\textsc{StudentPrompt}$ presents the problem and $\textsc{TeacherPrompt}$ prepends the blueprint (templates in Appendix~\ref{app:prompt_templates}). The two evaluations share everything---model, reference tokens, autoregressive factorization---except the blueprint in the teacher prefix. The student branch receives gradient; the teacher branch is detached.

\paragraph{Step 3: The log-ratio estimates structural salience.}
The log-ratio of the two probabilities,
\begin{equation}
A_t^{\mathrm{ref}}
:=
\log p_T^t - \log p_S^t
= \log \frac{\pi_\theta(y_t^\star \mid \textsc{TeacherPrompt}, y_{<t}^\star)}{\pi_\theta(y_t^\star \mid \textsc{StudentPrompt}, y_{<t}^\star)},
\label{eq:proxy_adv}
\end{equation}
is exactly the plug-in estimator of $\sigma_t$ with the blueprint $\hat{y}$ substituting for the true plan $S$: $A_t^{\mathrm{ref}} = \hat{\sigma}_t$. A large positive $A_t^{\mathrm{ref}}$ means the blueprint makes the token substantially easier to predict, indicating strong structural dependence.

\subsection{Token Weighting via the Geometric Mean}

We build on DFT~\citep{wu2026generalizationsftreinforcementlearning}, which stabilizes reference-path learning via $\mathcal{L}_{\mathrm{DFT}} = -\sum_t \operatorname{sg}(p_S^t)\log p_S^t$, but weights all tokens uniformly. To inject structural selectivity, we replace the DFT weight $p_S^t$ with the following construction.

\paragraph{From oracle to SOLD weight.}
An oracle with access to the true plan $S$ would use weight $\omega_t^\star = \operatorname{sg}(p_S^t \cdot e^{\beta\sigma_t})$ with $\beta \in [0,1]$, which exceeds the DFT baseline $p_S^t$ exactly when $\sigma_t > 0$. Substituting the estimated salience $A_t^{\mathrm{ref}}$ for $\sigma_t$ and the blueprint $\hat{y}$ for $S$ yields the SOLD weight family:
\begin{equation}
\boxed{\;
\omega_{\beta,t}
=
\operatorname{sg}\!\left(p_S^t \cdot e^{\beta A_t^{\mathrm{ref}}}\right)
\;=\;
\operatorname{sg}\!\left((p_S^t)^{1-\beta} (p_T^t)^\beta\right).
\;}
\label{eq:weight_family}
\end{equation}
The intuition is straightforward: if revealing the blueprint makes a token much easier to predict ($A_t^{\mathrm{ref}} \gg 0$), that token likely encodes a reasoning step the student has not yet mastered and deserves higher learning weight. If the blueprint offers no help ($A_t^{\mathrm{ref}} \approx 0$), the token is either already well-learned or superficial, and the weight falls back to DFT. We use $\beta = \tfrac{1}{2}$, the geometric mean $\omega_t = \operatorname{sg}(\sqrt{p_S^t p_T^t})$, which balances the two signals symmetrically. \begin{lemma}[Blueprint-regret bound]
\label{lem:regret}
Assume $|\log p_T^t - \log \pi_\theta(y_t^\star \mid S, y_{<t}^\star, q)| \le \delta$ for all $t$. Then $|\omega_t - \omega_t^\star| \le \frac{\delta}{2}\sqrt{p_S^t} \le \frac{\delta}{2}$. As $\delta \to 0$, the SOLD weight converges to the oracle; the error is suppressed on tokens with $\sqrt{p_S^t} \ll 1$. Proof in Appendix~\ref{sec:regret_bound}.
\end{lemma}

\paragraph{What the gradient reveals.}
Since the weights are detached, differentiating the auxiliary loss is straightforward. For a single token with weight $\omega = \operatorname{sg}(p_S \cdot e^{\beta A_t^{\mathrm{ref}}})$:
\begin{equation}
-\nabla_\theta\bigl(\omega \log p_S\bigr)
= -\omega \cdot \frac{\nabla_\theta p_S}{p_S}
= -\operatorname{sg}\!\left(e^{\beta A_t^{\mathrm{ref}}}\right)\nabla_\theta p_S
= -\operatorname{sg}\!\left(\bigl(\tfrac{p_T}{p_S}\bigr)^\beta\right)\nabla_\theta p_S.
\label{eq:token_gradient}
\end{equation}
Relative to DFT, whose per-token gradient is $-\nabla_\theta p_S$, SOLD rescales each token's update by $\exp(\beta A_t^{\mathrm{ref}}) = (p_T/p_S)^\beta$. With $\beta=\tfrac{1}{2}$, a token whose probability doubles under blueprint conditioning ($p_T/p_S \approx 2$) receives $\approx$1.4$\times$ the DFT update; a token where the blueprint provides no help ($p_T/p_S \approx 1$) receives exactly the DFT update; a token where the blueprint reduces confidence ($p_T/p_S < 1$) is automatically downweighted.

\paragraph{Full auxiliary objective.}
Aggregating over a buffered minibatch $\mathcal{M}_k$ with token set $\mathcal{S}(\mathcal{M}_k)$:
\begin{equation}
\mathcal{L}_{\mathrm{SOLD}}(\mathcal{M}_k)
=
-\frac{1}{|\mathcal{S}(\mathcal{M}_k)|}
\sum_{(i,t) \in \mathcal{S}(\mathcal{M}_k)}
\omega_{\beta,t}
\log \pi_\theta\!\left(y_{i,t}^\star \;\middle|\; y_{i,<t}^\star,\, \mathbf{p}_i\right),
\label{eq:sold_loss}
\end{equation}
where only the student branch receives gradient.

\subsection{Interleaved Optimization}
\label{sec:loss}

SOLD and GRPO are applied as sequential updates: a GRPO step on the rollout batch, followed by a SOLD step on a buffered minibatch whenever $|\mathcal{B}_{\mathrm{aw}}| \ge B_{\mathrm{aux}}$. This decoupling keeps on-policy exploration separate from reference-supported repair. The complete procedure is Algorithm~\ref{alg:sold}.

\begin{algorithm}[t]
\caption{Interleaved GRPO with Buffered SOLD}
\label{alg:sold}
\begin{algorithmic}[1]
\REQUIRE Policy parameters $\theta$, batch size $B_{\mathrm{rl}}$, rollouts per prompt $N$, auxiliary batch size $B_{\mathrm{aux}}$, empty buffer $\mathcal{B}_{\mathrm{aw}}$
\FOR{$k = 1, \dots, K$}
    \STATE Sample rollout batch $\mathcal{U}_k = \{q_i\}_{i=1}^{B_{\mathrm{rl}}}$
    \FOR{$i = 1, \dots, B_{\mathrm{rl}}$}
        \STATE Sample $\{y_i^{(n)}\}_{n=1}^N \sim \pi_\theta(\cdot \mid q_i)$, compute rewards $\{r_i^{(n)}\}_{n=1}^N$
        \STATE Compute GRPO advantages
    \ENDFOR
    \STATE $\theta \leftarrow \operatorname{Update}_{\mathrm{GRPO}}(\theta; \mathcal{L}_{\mathrm{GRPO}}(\mathcal{U}_k))$
    \STATE $\mathcal{I}_{\mathrm{aw}}^{(k)} \gets \{ i \mid r_i^{(n)} = 0,\; \forall n \in [N] \}$
    \STATE Enqueue $\{(q_i, y_i^\star) : i \in \mathcal{I}_{\mathrm{aw}}^{(k)}\}$ into $\mathcal{B}_{\mathrm{aw}}$
    \IF{$|\mathcal{B}_{\mathrm{aw}}| \ge B_{\mathrm{aux}}$}
        \STATE Sample and remove $\mathcal{M}_k \sim \operatorname{SampleBatch}(\mathcal{B}_{\mathrm{aw}}, B_{\mathrm{aux}})$
        \FORALL{$(q_i, y_i^\star) \in \mathcal{M}_k$}
            \STATE $\hat{y}_i \gets \operatorname{Gen}_\theta(\textsc{SkelPrompt}(q_i, y_i^\star))$ \quad // extract reasoning structure
            \STATE Construct $\mathbf{p}_i$ (student) and $\mathbf{p}_i^{\mathrm{T}}$ (teacher with $\hat{y}_i$)
            \STATE Compute $\ell_{i,t}^{\mathrm{S}}, \ell_{i,t}^{\mathrm{T}}$ along $y_i^\star$ for all $t$
            \STATE $\omega_{i,t} \gets \operatorname{sg}\!\bigl(\sqrt{\exp(\ell_{i,t}^{\mathrm{S}}) \exp(\ell_{i,t}^{\mathrm{T}})}\,\bigr)$ for all $t$
        \ENDFOR
        \STATE $\theta \leftarrow \operatorname{Update}_{\mathrm{SOLD}}(\theta; \mathcal{L}_{\mathrm{SOLD}}(\mathcal{M}_k))$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

